Study of $B^0_s \rightarrow J/\psi\pi^+\pi^-K^+K^-$ decays

The decays $B^0_s \rightarrow J/\psi \pi^+\pi^- K^+ K^-$ are studied using a data set corresponding to an integrated luminosity of 9fb$^{-1}$, collected with the LHCb detector in proton-proton collisions at centre-of-mass energies of 7, 8 and 13TeV. The decays $B^0_s \rightarrow J/\psi K^{\ast0} \bar{K}^{\ast0}$ and $B^0_s \rightarrow \chi_{c1}(3872)K^+K^-$, where the $K^+K^-$ pair does not originate from a $\phi$ meson, are observed for the first time. Precise measurements of the ratios of branching fractions between intermediate $\chi_{c1}(3872)\phi$, $J/\psi K^{\ast0}\bar{K}^{\ast0}$, $\psi(2S)\phi$ and $\chi_{c1}(3872)K^+K^-$ states are reported. A structure, denoted as $X(4740)$, is observed in the $J/\psi\phi$ mass spectrum and, assuming a Breit-Wigner parameterisation, its mass and width are determined to be \begin{eqnarray*} m_{X(4740)} & = & 4741 \pm 6 \pm 6\,{\mathrm{MeV}}/c^2 \,, \\ \Gamma_{X(4740)} & = & 53 \pm 15 \pm 11\,{\mathrm{MeV}} \,, \end{eqnarray*} where the first uncertainty is statistical and the second is systematic. In addition, the most precise single measurement of the mass of the $B^0_s$ meson is performed and gives a value of $$ m_{B^0_s} = 5366.98 \pm 0.07 \pm 0.13\,{\mathrm{MeV}}/c^2\,. $$

==> LHCb_Authorship_07-Sep-2020_arXiv.tex <==
LHCb collaboration:
R. Aaij,
C. Abell{\'a}n Beteta,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
S. Amato,
Y. Amhis,
L. An,
L. Anderlini,
A. Andreianov,
M. Andreotti,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
S. Baker,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista Leite,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Battig,
A. Bay,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
S. Bifani,
P. Billoir,
M. Birch,
F.C.R. Bishop,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
L. Calero Diaz,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
A. Camboni,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
L. Carus,
K. Carvalho Akiba,
A. Casais Vidal,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
J. Cerasoli,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
S.-G. Chitic,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
J.A. de Vries,
C.T. Dean,
W. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
A. Dendek,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
H. Dijkstra,
V. Dobishuk,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
K. Dreimanis,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
A. Falabella,
J. Fan,
Y. Fan,
B. Fang,
N. Farley,
S. Farry,
D. Fazzini,
P. Fedin,
M. F{\'e}o,
P. Fernandez Declara,
A. Fernandez Prieto,
J.M. Fernandez-tenllado Arribas,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
W. Funk,
E. Gabriel,
T. Gaintseva,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
L. Giubega,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
P. Griffith,
L. Grillo,
S. Gromov,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
T. Halewood-leagas,
P.M. Hamilton,
Q. Han,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
J. Hu,
J. Hu,
W. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
M. Jezabek,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
N. Kazeev,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
K.E. Kim,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
L. Li,
P. Li,
X. Li,
Y. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
S. Liu,
X. Liu,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
G. Loustau,
G.H. Lovell,
Y. Lu,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Madejczyk,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
R. Manera Escalero,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
P.J. Marshall,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
G. Meier,
N. Meinert,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
L. Minzoni,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden,
R.A. Mohammed,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mukherjee,
M. Mulder,
D. M{\"u}ller,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
I. Neri,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
D.P. O'Hanlon,
R. Oldeman,
M.E. Olivares,
C.J.G. Onderwater,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
C.J. Parkinson,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
T.T.H. Pham,
A. Philippov,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
F. Pisani,
A. Piucci,
Resmi  P.K,
V. Placinta,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
S. Ricciardi,
D.S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
D. Sanchez Gonzalo,
C. Sanchez Gras,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
P. Seyfert,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
V. Shevchenko,
E.B. Shields,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
G. Simi,
S. Simone,
I. Skiba,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
J.G. Smeaton,
A. Smetkina,
E. Smith,
M. Smith,
A. Snoch,
M. Soares,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
H. Stevens,
S. Stone,
M.E. Stramaglia,
M. Straticiuc,
D. Strekalina,
S. Strokov,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
F. Teubert,
E. Thomas,
K.A. Thomson,
M.J. Tilley,
V. Tisserand,
S. T'Jampens,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Torres Machado,
D.Y. Tou,
M. Traill,
M.T. Tran,
E. Trifonova,
C. Trippl,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D. Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
P. Vincent,
G. Vitali,
A. Vollhardt,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
H.M. Wark,
N.K. Watson,
S.G. Weber,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
D. Wiedner,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhou,
Y. Zhou,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli,
D. Zuliani,
G. Zunica

==> old_plots.tex <==
 	
\begin{figure}[t]
  \setlength{\unitlength}{1mm}
  \centering
  \begin{picture}(150,130)
    %% 
    %% \graphpaper[5](-10,-10)(170,140)
    %% 
    %
    \put(  0, 60){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/x_3D_Bs_sim.pdf}
    }
     \put( 75, 60){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/x_3D_phi_sim.pdf}
    }
    \put(  0,  0){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/x_3D_x_sim.pdf}
    }
    %% Candidates$/(5\,\mevcc)
    \put( 2 , 95){\rotatebox[]{90} {Candidates$/(5\mevcc)$} }
    \put( 76, 95) {\rotatebox[]{90}{Candidates$/(4\mevcc)$} }
    \put(  2, 35) {\rotatebox[]{90}{Candidates$/(1\mevcc)$} }
    %% 
    \put( 25, 60) { $m_{\jpsi\Kp\Km\pip\pim}$} \put( 57,60) { $\left[\!\gevcc\right]$} 
    \put(110, 60) { $m_{\Kp\Km}$} \put(132,60) { $\left[\!\gevcc\right]$} 
    \put( 35,  0) { $m_{\jpsi\pip\pim}$} \put( 57, 0) { $\left[\!\gevcc\right]$} 
    %% 
    
	\put( 17,53){\scriptsize$5.35<m_{\jpsi\pip\pim\Kp\Km}<5.39\gevcc$}
	\definecolor{gr}{rgb}{0.35, 0.83, 0.33}
	\definecolor{db}{rgb}{0.1, 0.08, 0.41}
	 \put(90,50) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=red!35!white,draw=red,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,45){\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=gray!35!white,draw=gray,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,40){\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=blue!35!white,draw=blue,thick]    (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,35) {\begin{tikzpicture}[x=1mm,y=1mm]    \draw[thin,gr,pattern=north east lines, pattern color=gr]  (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,30) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=gr!35!white,draw=gr,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,25)
	{\begin{tikzpicture}[x=1mm,y=1mm]	\draw[thin,gray,pattern=north west lines, pattern color=gray]    (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,20) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=db!75!white,draw=db,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,15) {\color[RGB]{26,21,104}     {\hdashrule[0.0ex][x]{8mm}{1.0pt}{2.0mm 0.3mm} } }
	\put(90,10){\color[RGB]{255,153,51} {\rule{8mm}{2.0pt}}}
	
	\put( 100,50){\small{\decay{\Bs}{\chicone(3872)\Pphi}}}
	\put( 100,45){\small{\decay{\Bs}{\left(\jpsi\pip\pim\right)_{\cancel{\PX_{\ccbar}}}\Pphi}}}
	\put( 100,40){\small{\decay{\Bs}{\chicone(3872) \left(\Kp\Km\right)_{\cancel{\Pphi}}}}}
	\put( 100,35){\small{\decay{\Bs}{\jpsi\Kp\Km\pip\pim }}}

	\put( 100,30){\small{comb. $\chicone(3872)\Pphi$}}
	\put( 100,25){\small{comb. $\left(\jpsi\pip\pim\right)_{\cancel{\PX_{\ccbar}}}\Pphi$}}
	\put( 100,20){\small{comb. $\chicone(3872) \left(\Kp\Km\right)_{\cancel{\Pphi}}$}}

	\put( 100,15){\small{comb. $\jpsi\Kp\Km\pip\pim$}} 
	\put( 100,10){\small{total}}
  \end{picture}
  \caption { \small
   Distributions 
   of the~(top left)~\mbox{$\jpsi\Kp\Km\pip\pim$},
   (top right)~\mbox{$\Kp\Km$} and 
   (bottom left)~\mbox{$\jpsi\pip\pim$}~mass
   of selected \mbox{$\decay{\Bs}{\chicone(3872)\Pphi}$}~candidates
   shown as points with error bars. 
   A~fit, described in the~text, is overlaid.
  }
  \label{fig:fit_sim_chi}
\end{figure}


\begin{figure}[t]
  \setlength{\unitlength}{1mm}
  \centering
  \begin{picture}(150,130)
    %% 
    %% \graphpaper[5](-10,-10)(170,140)
    %% 
    %
    \put(  0, 60){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/psi_3D_Bs_sim.pdf}
    }
     \put( 75, 60){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/psi_3D_phi_sim.pdf}
    }
    \put(  0,  0){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/psi_3D_psi_sim.pdf}
    }
    %% Candidates$/(5\,\mevcc)
    \put( 2 , 95){\rotatebox[]{90} {Candidates$/(5\mevcc)$} }
    \put( 76, 95) {\rotatebox[]{90}{Candidates$/(4\mevcc)$} }
    \put(  2, 35) {\rotatebox[]{90}{Candidates$/(1\mevcc)$} }
    %% 
    \put( 25, 60) { $\MBs$} \put( 57,60) { $\left[\!\gevcc\right]$} 
    \put(110, 60) { $\Mphi$} \put(132,60) { $\left[\!\gevcc\right]$} 
    \put( 35,  0) { $\Mpsi$} \put( 57, 0) { $\left[\!\gevcc\right]$} 
    %% 
    
  
	\definecolor{gr}{rgb}{0.35, 0.83, 0.33}
	\definecolor{db}{rgb}{0.1, 0.08, 0.41}

	 \put(90,50) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=red!35!white,draw=red,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,45){\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=gray!35!white,draw=gray,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,40){\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=blue!35!white,draw=blue,thick]    (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,35) {\begin{tikzpicture}[x=1mm,y=1mm]    \draw[thin,gr,pattern=north east lines, pattern color=gr]  (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,30) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=gr!35!white,draw=gr,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,25)
	{\begin{tikzpicture}[x=1mm,y=1mm]	\draw[thin,gray,pattern=north west lines, pattern color=gray]    (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,20) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=db!75!white,draw=db,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
	\put(90,15) {\color[RGB]{26,21,104}     {\hdashrule[0.0ex][x]{8mm}{1.0pt}{2.0mm 0.3mm} } }
	\put(90,10){\color[RGB]{255,153,51} {\rule{8mm}{2.0pt}}}
	\put( 17,53){\scriptsize$5.35<m_{\jpsi\pip\pim\Kp\Km}<5.39\gevcc$}
	\put( 100,50){\small{\decay{\Bs}{\psitwos\Pphi}}}
	\put( 100,45){\small{\decay{\Bs}{\left(\jpsi\pip\pim\right)_{\cancel{\PX_{\ccbar}}}\Pphi}}}
	\put( 100,40){\small{\decay{\Bs}{\psitwos \left(\Kp\Km\right)_{\cancel{\Pphi}}}}}
	\put( 100,35){\small{\decay{\Bs}{ \jpsi\Kp\Km\pip\pim }}}

	\put( 100,30){\small{comb. $\psitwos\Pphi$}}
	\put( 100,25){\small{comb. $\left(\jpsi\pip\pim\right)_{\cancel{\PX_{\ccbar}}}\Pphi$}}
	\put( 100,20){\small{comb. $\psitwos \left(\Kp\Km\right)_{\cancel{\Pphi}}$}}

	\put( 100,15){\small{comb. $\jpsi\Kp\Km\pip\pim$ }}
	\put( 100,10){\small{total}}
  \end{picture}
  \caption { \small
   Mass distributions of the selected $\BsTopsitwophi$ candidates\,(points with error bars).  The~fit, described in the text, is overlaid.
  }
  \label{fig:fit_sim_psi}
\end{figure}

\begin{figure}[t]
  \setlength{\unitlength}{1mm}
  \centering
  \begin{picture}(150,60)
    \put(  0, 0){ 
      \includegraphics*[width=75mm,height=60mm,%
      ]{figs/Bs_XKK_fit_2D.pdf}
    }
     \put( 75, 00){ 
      \includegraphics*[width=75mm,height=60mm,%
      ]{figs/x_XKK_fit_2D.pdf}
    }
    \put( 75, 32) {\rotatebox[]{90}{Candidates$/(1\mevcc)$} }
    \put(  -2,32) {\rotatebox[]{90}{Candidates$/(5\mevcc)$} }
    \put(105, 0) { $m_{\jpsi\pip\pim}$} \put(132,0) { $\left[\!\gevcc\right]$} 
    \put( 30,  0) { $m_{\jpsi\Kp\Km\pip\pim}$} \put( 57, 0) { $\left[\!\gevcc\right]$} 

    \put(133,51){\small\lhcb}
    \put(58,51){\small\lhcb}
	%% f
    \put(38,45) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=red!35!white,draw=red,thick]  (0,0) rectangle (5,3);\end{tikzpicture} }
	\put(38,41) {\color[RGB]{121,220,117}     {\rule{6mm}{2.0pt}}}
	\put(38,36) {\color[RGB]{118,118,118}     {\hdashrule[0.0ex][x]{6mm}{1.0pt}{2.0mm 0.3mm} } }
	\put(38,31){\color[RGB]{85,83,246}     {\hdashrule[0.0ex][x]{6mm}{1.0pt}{2.0mm 0.3mm} } }
	\put(38,26){\color[RGB]{255,153,51} {\rule{6mm}{2.0pt}}}

	%%
	\put( 45,46){\scalebox{0.8}{\tiny{\decay{\Bs}{\chicone(3872) \Km\Kp}}}}
	\put( 45,41){\scalebox{0.8}{\tiny{\decay{\Bs}{\left(\jpsi \pip \pim \Kp \Km\right)_{\mathrm{NR}}}}}}
	\put( 45,36){\scalebox{0.8}{\tiny{comb.$\chicone(3872) \Km\Kp$}}}
	\put( 45,31){\scalebox{0.8}{\tiny{comb.$\jpsi\pip\pim\Kp\Km$}}}
	\put( 45,26){\scalebox{0.8}{\tiny{total}}}
	%%


  \end{picture}
	\caption{\small 
	Distributions of 
	the~(left)~$\jpsi\Kp\Km\pip\pim$ and 
	(right)~$\jpsi\pip\pim$~mass of 
	selected $\decay{\Bs}{\chicone(3872)\Kp\Km}$ candidates shown as points with error bars.
	A~fit, described in the~text, is overlaid.}
	\label{fig:fit_XKK}
\end{figure}
 
 


\begin{figure}[t]
  \setlength{\unitlength}{1mm}
  \centering
    \begin{picture}(150,60)
    \put(  0, 0){ 
      \includegraphics*[width=75mm,height=60mm,%
      ]{figs/phi_XKK_fit_1D.pdf}
    }
     \put( 75, 00){ 
      \includegraphics*[width=75mm,height=60mm,%
      ]{figs/phi_XKK_fit_1D_zoom.pdf}
    }
    \put( 75, 32) {\small\rotatebox[]{90}{$N_{\decay{\Bs}{\chicone(3872)\Kp\Km}}/(15\mevcc)$} }
    \put(  -2,32) {\small\rotatebox[]{90}{$N_{\decay{\Bs}{\chicone(3872)\Kp\Km}}/(30\mevcc)$} }
    \put(105, 0) { $m_{\Kp\Km}$} \put(132,0) { $\left[\!\gevcc\right]$} 
    \put( 30,  0) { $m_{\Kp\Km}$} \put( 57, 0) { $\left[\!\gevcc\right]$} 
    \put(133,51){\small\lhcb}
    \put(58,51){\small\lhcb}

   \put( 92,50) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=red!35!white,draw=red,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }

	\put(92,46){\color[RGB]{85,83,246}     {\hdashrule[0.0ex][x]{8mm}{1.0pt}{2.0mm 0.3mm} } }
	\put(92,41){\color[RGB]{255,153,51} {\rule{8mm}{2.0pt}}}
   \put( 92,36){\color[RGB]{121,220,117} {\rule{8mm}{2.0pt}}}
   
   %% \put(92,45) {\color[RGB]{98,210,54}     {\hdashrule[0.0ex][x]{8mm}{1.0pt}{2.0mm 0.3mm} } }
   
	%%
	\put( 101,51){{\scriptsize{\decay{\Bs}{\chicone(3872) \Pphi}}}}
	\put( 101,46){{\scriptsize{\decay{\Bs}{\chicone(3872)\left( \Kp\Km\right)_{\cancel{\Pphi}}}}}} 
	\put( 101,41){{\scriptsize{total}}}
	%% 
	\put( 101,36){{\scriptsize{simulation}}}

  \end{picture}
 	\caption{\small 
 	%%
 	Background-subtracted and corrected for the~$\Kp\Km$~mass-dependent 
 	efficiency
 	$\Kp\Km$~mass distribution (points with error bars) 
    from 
    the~$\mbox{$\decay{\Bs}{\chicone(3872)\Kp\Km}$}$~decays.
    For~better 
 	%% for~(left)~the~full range 
 	%%and (right) zoomed for 
 	%% better 
 	visualization 
 	of the~high mass region
 	the~right plot is shown with zoomed vertical scale.
 	A~fit, described in the~text, is superimposed on the~right~plot.
 	An~expectation for phase\nobreakdash-space
 	simulated decays
    is shown as green solid line. 
    %%
    %% The~efficiency is normalized to unity at the~known mass of the~\Pphi~meson.
    }
	\label{fig:KK_mss}
\end{figure}

 
 
 \begin{figure}[tb]
  \setlength{\unitlength}{1mm}
  \centering
  \begin{picture}(150,130)
    %% 
    %% \graphpaper[5](-10,-10)(170,140)
    %% 
    %
    \put(  0, 60){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/ks_fit_3D_Bs.pdf}
    }
     \put( 75, 60){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/ks_fit_3D_ks.pdf}
    }
    \put(  0,  0){ 
      \includegraphics*[width=75mm,height=60mm,%
      %%]{DD_mass.pdf}
      ]{figs/ks_fit_3D_ksb.pdf}
    }
    %% Candidates$/(5\,\mevcc)
    \put( 3 , 95){\rotatebox[]{90} {Candidates$/(5\mevcc)$} }
    \put( 76, 95) {\rotatebox[]{90}{Candidates$/(10\mevcc)$} }
    \put(  2, 35) {\rotatebox[]{90}{Candidates$/(10\mevcc)$} }
    %% 
    \put( 25, 60) { $m_{\jpsi\Kp\Km\pip\pim}$} \put( 57,60) { $\left[\!\gevcc\right]$} 
    \put(110, 60) { $m_{\Kp\pim}$} \put(132,60) { $\left[\!\gevcc\right]$} 
    \put( 35,  0) { $m_{\Km\pip}$} \put( 57, 0) { $\left[\!\gevcc\right]$} 
    %% 
    
    
    \definecolor{gr}{rgb}{0.35, 0.83, 0.33}
	\definecolor{db}{rgb}{0.1, 0.08, 0.41}

	\put( 58,51){\small\lhcb}
	\put( 58,111){\small\lhcb}
	\put( 133,111){\small\lhcb}

	 \put(90,50) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=red!35!white,draw=red,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,45) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=gray!35!white,draw=gray,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,40){\begin{tikzpicture}[x=1mm,y=1mm]\draw[thin,gr,pattern=north east lines, pattern color=gr]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,35) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=db!35!white,draw=db,thick]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,30){\begin{tikzpicture}[x=1mm,y=1mm]\draw[thin,db,pattern=north west lines, pattern color=db]  (0,0) rectangle (8,3);\end{tikzpicture} }
    \put(90,25){\color[RGB]{85,83,246}     {\hdashrule[0.0ex][x]{8mm}{1.0pt}{2.0mm 0.3mm} } }
	\put(90,20){\color[RGB]{255,153,51} {\rule{8mm}{2.0pt}}}
	\put( 100,51){\small{\decay{\Bs}{\jpsi \Kstarz \Kstarzb}}}
	\put( 100,46){\small{\decay{\Bs}{\jpsi\Kstar \left(\kaon \pion \right)_{\cancel{\Kstar}}}}}
    \put( 100,41){\small{\decay{\Bs}{\jpsi\pip\pim\Kp\Km}}}
	\put( 100,35){\small comb. $\jpsi \Kstarz \Kstarzb$}
	\put( 100,30){\small comb. $\jpsi\Kstar \left(\kaon \pion \right)_{\cancel{\Kstar}}$}

	\put( 100,25){\small{comb. bkg.}}
	\put( 100,20.05){\small{total}}
  \end{picture}
  \caption { \small
   Distributions of 
   the~(top left)~\mbox{$\jpsi\Kp\Km\pip\pim$},
   (top right)~\mbox{$\Kp\pim$}
   and 
   (bottom left)~\mbox{$\Km\pip$}
   mass of selected $\BsTokstkst$ candidates 
   shown as points with error bars.   
   A~fit, described in the~text, is overlaid.
  }
  \label{fig:fit_kstar}
\end{figure}

 
 

\begin{figure}[t]
  \setlength{\unitlength}{1mm}
  \centering
  \begin{picture}(150,120)
    %% 
    %% \graphpaper[5](-10,-10)(170,140)
    %% 
    %
    %\newcommand{\cross}[1][2.5]{
    %\begin{tikzpicture}[x=1ex, y=1ex, scale=#1]
     %   \draw[thick] (-0.3,  0)  -- (0.3, 0);
      %  \draw[thick] (0,  0.4)  -- (0, -0.4);
      %  \fill [color=red] (0,0) circle (0.1);
    %\end{tikzpicture}
    %}
    \put(0, 0){ 
      \includegraphics*[width=150mm,height=120mm,%
       %%]{DD_mass.pdf}
       ]{figs/x4700_base.pdf}
    }
    %%
    \put(2,55) {\large\begin{sideways}$N_{\BsTopsiphtwopi}/(15\mevcc)$\end{sideways}}
    \put(120,102){\Large\lhcb}
    %%
   \put(40,100) {\begin{tikzpicture}[x=1mm,y=1mm]\filldraw[fill=red!35!white,draw=red,thick]  (0,0) rectangle (13,3);\end{tikzpicture} }
    %%
	\put(40,94){\color[RGB]{85,83,246}     {\hdashrule[0.0ex][x]{13mm}{1.0pt}{2.0mm 0.5mm} } }
	%%
	\put(40,88){\color[RGB]{255,153,51} {\rule{13mm}{2.0pt}}}
	%%
	\put(55,100){$\decay{\Bs}{\PX(4370)\pip\pim}$}
	\put( 55,94){\decay{\Bs}{\jpsi \pip \pim \Pphi}}
	\put( 55,88){total}
    %% 
    \put( 65,2){\Large{$m_{\jpsi\Pphi}$}}
    \put(125,2){\Large{$\left[\!\gevcc\right]$}}
    %% 
  \end{picture}
	\caption{\small 
	Background-subtracted $\jpsi\Pphi$~mass 
	distribution from 
	\mbox{$\BsTopsiphtwopi$}~decays\,(points with error bars)
	A~fit, described in 
	the~text, is
	superimposed.}
	\label{fig:xxx_fit}

\end{figure}
